Scalable Pseudorandom Quantum States

Efficiently sampling a quantum state that is hard to distinguish from a truly random quantum state is an elementary task in quantum information theory that has both computational and physical uses. This is often referred to as pseudorandom (quantum) state generator, or PRS generator for short. In existing constructions of PRS generators, security scales with the number of qubits in the states, i.e.\ the (statistical) security parameter for an $n$-qubit PRS is roughly $n$. Perhaps counter-intuitively, $n$-qubit PRS are not known to imply $k$-qubit PRS even for $k<n$. Therefore the question of \emph{scalability} for PRS was thus far open: is it possible to construct $n$-qubit PRS generators with security parameter $\lambda$ for all $n, \lambda$. Indeed, we believe that PRS with tiny (even constant) $n$ and large $\lambda$ can be quite useful. We resolve the problem in this work, showing that any quantum-secure one-way function implies scalable PRS. We follow the paradigm of first showing a \emph{statistically} secure construction when given oracle access to a random function, and then replacing the random function with a quantum-secure (classical) pseudorandom function to achieve computational security. However, our methods deviate significantly from prior works since scalable pseudorandom states require randomizing the amplitudes of the quantum state, and not just the phase as in all prior works. We show how to achieve this using Gaussian sampling.

==> appx.tex <==

\section{Proofs from Section~\ref{subsec:gaussian}}
\label{sec:appendix}

In this subsection we provide the formal proofs the lemmas from Section~\ref{subsec:gaussian} that support the proof of Theorem \ref{thm:main}, which describe properties of the multidimensional Gaussian distribution.

\subsection{Proof of Lemma \ref{lemma:gaussian_vectors_coordinate_bounded}}

\begin{proof}
	The proof follows by a calculation and by known properties of the Gaussian distribution.
	$$
	\Pr_{v \gets \normalCompDist^{2^n}}\Big[ \exists i \in [2^n] : |v_i| > B \Big] \underset{(\text{union bound})}{\leq}
	2^n \cdot \Pr_{z \gets \normalCompDist}\Big[ |z| > B \Big] = 
	$$
	$$
	2^n \cdot \Pr_{y \gets \normalDist^2}\Big[ \sqrt{y^2_1 + y^2_2} > B \Big] \underset{(\text{union bound})}{\leq}
	2^n \cdot 2 \cdot \Pr_{x \gets \normalDist}\bigg[ |x| > \frac{B}{\sqrt{2}} \bigg] =
	$$
	$$
	2^n \cdot 4\cdot \Pr_{x \gets \normalDist}\bigg[ x > \frac{B}{\sqrt{2}} \bigg]\underset{(*)}{<}
	$$
	$$
	2^{n} \cdot 4\cdot \frac{1}{B\sqrt{\pi}} \cdot e^{-\frac{B^2}{2}\cdot \frac{1}{2}} = 
	\frac{4}{B \sqrt{\pi}} \cdot 2^{n} \cdot e^{-\frac{B^2}{4}} \underset{\left( B \geq 2\cdot \sqrt{n + \secp} \right)}{<} 
	e^{- \secp} \enspace ,
	$$
	where $(*)$ follows from a well known upper bound on the q-function of the Gaussian distribution:
	$$
	\forall t \geq 0 : \Pr_{x \gets \normalDist}\big[ x > t \big] < \frac{1}{t\sqrt{2\cdot \pi}} \cdot e^{-\frac{t^2}{2}} \enspace .
	$$
\end{proof}

\subsection{Proof of Corollary \ref{lemma:gaussian_vectors_balanced}}

\begin{proof}
	$$
	1 - e^{-\frac{2^n}{4}} \leq 
	1 - e^{-\left( \frac{7}{8} \right)^2 \cdot \frac{2\cdot 2^n}{4}}
	\underset{(\text{Lemma \ref{lemma:gaussian_vectors_long}})}{\leq}
	\Pr_{u \gets \normalDist^{2\cdot 2^n}}\left[ \norm{u}^2 \geq \left( 1 - \frac{7}{8} \right)\cdot \left( 2\cdot 2^n \right) \right] = 
	$$
	$$
	\Pr_{u \gets \normalDist^{2\cdot 2^n}}\left[ \norm{u} \geq \frac{\sqrt{2^n}}{2} \right] = 
	\Pr_{v \gets \normalCompDist^{2^n}}\left[ \norm{v} \geq \frac{\sqrt{2^n}}{2} \right] = 
	$$
	$$
	\Pr_{v \gets \normalCompDist^{2^n}}\left[ \left( \norm{v} \geq \frac{\sqrt{2^n}}{2} \right) \land \left( \exists i \in [2^n] : |v_i| > B \right) \right] + 
	$$
	$$
	\Pr_{v \gets \normalCompDist^{2^n}}\left[ \left( \norm{v} \geq \frac{\sqrt{2^n}}{2} \right) \land \left( \forall i \in [2^n] : |v_i| \leq B \right) \right] \leq
	$$
	$$
	\Pr_{v \gets \normalCompDist^{2^n}}\Big[ \exists i \in [2^n] : |v_i| > B \Big] + 
	$$
	$$
	\Pr_{v \gets \normalCompDist^{2^n}}\left[ \left( \norm{v} \geq \frac{\sqrt{2^n}}{2} \right) \land \left( \forall i \in [2^n] : |v_i| \leq B \right) \right] \underset{(\text{Lemma }\ref{lemma:gaussian_vectors_coordinate_bounded})}{<}
	$$
	$$
	e^{-\secp} +
	\Pr_{v \gets \normalCompDist^{2^n}}\left[ \left( \norm{v} \geq \frac{\sqrt{2^n}}{2} \right) \land \left( \forall i \in [2^n] : |v_i| \leq B \right) \right] \enspace ,
	$$
	
	and the above inequalities imply our wanted inequality,
	$$
	1 - \left( e^{-\frac{2^n}{4}} + e^{-\secp} \right) <
	\Pr_{v \gets \normalCompDist^{2^n}}\left[ \left( \norm{v} \geq \frac{\sqrt{2^n}}{2} \right) \land \left( \forall i \in [2^n] : |v_i| \leq B \right) \right] \enspace .
	$$
\end{proof}

\subsection{Proof of Corollary \ref{lemma:rounded_gaussian_vectors_long}}

\begin{proof}
	The calculation of the probability follows.
	$$
	\Pr_{v \gets \distribution{2^n}{\varepsilon, B}}\left[ \norm{v} \geq \frac{\sqrt{2^n}}{2} \right] = 
	\Pr_{u \gets \normalCompDist^{2^n}}\left[ \norm{R_{(\varepsilon, B)}(u)} \geq \frac{\sqrt{2^n}}{2} \right] \underset{(*)}{\geq}
	$$
	$$
	\Pr_{u \gets \normalCompDist^{2^n}}\left[ \left( \norm{u} \geq \frac{\sqrt{2^n}}{2} \right) \land \big( \forall i \in \left[ 2^n \right] : |u_i| \leq B \big) \right] \underset{(\text{Corollary }\ref{lemma:gaussian_vectors_balanced})}{>} 
	1 - \left( e^{-\frac{2^n}{4}} + e^{-\secp} \right) \enspace ,
	$$
	where $(*)$ is due to properties of the rounding function; if $|u_i| \leq B$ then in particular $\abs{\text{Re}(u_i)} \leq B$, $\abs{\text{Im}(u_i)} \leq B$, and then it is necessarily the case that $\forall i \in [2^n] : |u_i| \leq |R_{(\varepsilon, B)}(u_i)|$ which then implies $\norm{u} \leq \norm{R_{(\varepsilon, B)}(u)}$, and thus $\frac{\sqrt{2^n}}{2} \leq \norm{R_{(\varepsilon, B)}(u)}$ follows from $\frac{\sqrt{2^n}}{2} \leq \norm{u}$.
\end{proof}

%\begin{corollary} \label{cor:conditional_vectors_coordinates_bounded}
%	Let $n \in \bbN$, $\secp \in \bbN$ s.t. $\secp \geq 3$, $\varepsilon > 0$, $B \geq 2\sqrt{n + \secp}$ and let $D$ be the conditional distribution of $v \gets \normalCompDist^{2^n}$ with the condition that $\norm{R_{(\varepsilon, B)}(v)} \geq \frac{\sqrt{2^n}}{2}$.
%	Then,
%	$$
%	\Pr_{v \gets D}\Big[ \exists i \in [2^n] : |v_i| > B \Big] < 4 \cdot e^{-\secp} \enspace .
%	$$
%\end{corollary}

\subsection{Proof of Corollary \ref{cor:conditional_vectors_coordinates_bounded}}

\begin{proof}
	We have,
	$$
	e^{-\secp} \underset{(\text{Lemma }\ref{lemma:gaussian_vectors_coordinate_bounded})}{>}
	\Pr_{v \gets \normalCompDist^{2^n}}\Big[ \exists i \in [2^n] : |v_i| > B \Big] > 
	$$
	$$
	\Pr_{v \gets \normalCompDist^{2^n}}\bigg[ \bigg( \norm{R_{(\varepsilon, B)}(v)} \geq \frac{\sqrt{2^n}}{2} \bigg) \land \big( \exists i \in [2^n] : |v_i| > B \big) \bigg] = 
	$$
	$$
	\Pr_{v \gets \normalCompDist^{2^n}}\bigg[ \norm{R_{(\varepsilon, B)}(v)} \geq \frac{\sqrt{2^n}}{2} \bigg] \cdot
	\Pr_{v \gets D}\Big[ \exists i \in [2^n] : |v_i| > B \Big] = 
	$$
	$$
	\Pr_{u \gets \distribution{2^n}{\varepsilon, B}}\bigg[ \norm{u} \geq \frac{\sqrt{2^n}}{2} \bigg] \cdot
	\Pr_{v \gets D}\Big[ \exists i \in [2^n] : |v_i| > B \Big] \underset{(\text{Corollary }\ref{lemma:rounded_gaussian_vectors_long})}{>}
	$$
	$$
	\Big( 1 - \left( e^{-\frac{2^n}{4}} + e^{-\secp} \right) \Big) \cdot \Pr_{v \gets D}\Big[ \exists i \in [2^n] : |v_i| > B \Big] \underset{(2^n \geq 2 \; , \; \secp \geq 3)}{\geq}
	$$
	$$
	\Big( 1 - \left( e^{-\frac{1}{2}} + e^{-3} \right) \Big) \cdot \Pr_{v \gets D}\Big[ \exists i \in [2^n] : |v_i| > B \Big] >
	\left( \frac{3}{10} \right) \cdot \Pr_{v \gets D}\Big[ \exists i \in [2^n] : |v_i| > B \Big] \enspace .
	$$
	The above implies in particular,
	$$
	e^{-\secp} \cdot \left( \frac{10}{3} \right) > \Pr_{v \gets D}\Big[ \exists i \in [2^n] : |v_i| > B \Big] \enspace ,
	$$
	which implies our wanted inequality.
\end{proof}

%\begin{corollary} \label{cor:2nd_conditional_vectors_coordinates_bounded}
%	Let $n \in \bbN$, $\secp \in \bbN$, $\varepsilon > 0$, $B \geq 2\sqrt{n + \secp}$ and let $D$ be the conditional distribution of $v \gets \normalCompDist^{2^n}$ with the condition that $\norm{v} \geq \frac{\sqrt{2^n}}{2}$ (unlike the condition $\norm{R_{(\varepsilon, B)}(v)} \geq \frac{\sqrt{2^n}}{2}$ from Corollary \ref{cor:conditional_vectors_coordinates_bounded}).
%	Then,
%	$$
%	\Pr_{v \gets D}\Big[ \exists i \in [N] : |v_i| > B \Big] < 4\cdot e^{-\secp} \enspace .
%	$$
%\end{corollary}

\subsection{Proof of Corollary \ref{cor:2nd_conditional_vectors_coordinates_bounded}}

\begin{proof}
	We have,
	$$
	e^{-\secp} \underset{(\text{Lemma }\ref{lemma:gaussian_vectors_coordinate_bounded})}{>}
	\Pr_{v \gets \normalCompDist^{2^n}}\Big[ \exists i \in [2^n] : |v_i| > B \Big] > 
	$$
	$$
	\Pr_{v \gets \normalCompDist^{2^n}}\bigg[ \bigg( \norm{v} \geq \frac{\sqrt{2^n}}{2} \bigg) \land \big( \exists i \in [2^n] : |v_i| > B \big) \bigg] = 
	$$
	$$
	\Pr_{v \gets \normalCompDist^{2^n}}\bigg[ \norm{v} \geq \frac{\sqrt{2^n}}{2} \bigg] \cdot
	\Pr_{v \gets D}\Big[ \exists i \in [2^n] : |v_i| > B \Big] \underset{(\text{Lemma }\ref{lemma:gaussian_vectors_long})}{\geq}
	$$
	$$
	\Big( 1 - e^{-\frac{2^n}{4}} \Big) \cdot \Pr_{v \gets D}\Big[ \exists i \in [2^n] : |v_i| > B \Big] \underset{(2^n \geq 2)}{\geq}
	$$
	$$
	\Big( 1 - e^{-\frac{1}{2}} \Big) \cdot \Pr_{v \gets D}\Big[ \exists i \in [2^n] : |v_i| > B \Big] >
	\left( \frac{3}{10} \right) \cdot \Pr_{v \gets D}\Big[ \exists i \in [2^n] : |v_i| > B \Big] \enspace .
	$$
	The above implies in particular,
	$$
	e^{-\secp} \cdot \left( \frac{10}{3} \right) > \Pr_{v \gets D}\Big[ \exists i \in [2^n] : |v_i| > B \Big] \enspace ,
	$$
	which implies our wanted inequality.
\end{proof}

%\begin{lemma} [Long Vectors with Coordinate-Bounded Difference are Close \newline when Normalized] \label{lemma:long_vectors}
%	Let $n \in \bbN$, $0 \leq \varepsilon \leq \frac{1}{5}$ and $u, v \in \bbC^{2^n}$ s.t.
%	\begin{itemize}
%		\item 
%		$\norm{u} \geq \frac{\sqrt{2^n}}{2}$.
%		
%		\item 
%		$\forall i \in [2^n]: \abs{u_i - v_i} \leq \varepsilon$.
%	\end{itemize}
%	Then we have the following lower bound on the inner product of the unit vectors,
%	$$
%	\abs{\braket{u}{v}} \geq 1 - 18\cdot \varepsilon^2 \enspace .
%	$$
%\end{lemma}

\subsection{Proof of Lemma \ref{lemma:long_vectors}}

\begin{proof}
    Assume for this proof that whenever a vector is inside ket notation, it is implicitly normalized.
	We prove a lower bound for $\abs{\braket{u}{v}}$ by giving an upper bound on the distance between the normalizations $\norm{\ket{u} - \ket{v}}$.
	Intuitively, the geometric argument goes as follows:
	\begin{itemize}
		\item
		The distance $\norm{\ket{u} - \ket{v}}$ is exactly the distance between the two (un-normalized) vectors $u$ and $\frac{\norm{u}}{\norm{v}} \cdot v$, multiplied by the factor $\frac{1}{\norm{u}}$.
		We later use the fact that $u$ is very long, and thus the factor $\frac{1}{\norm{u}}$ will make the distance between the un-normalized vectors very small.
		
		\item
		The distance from $u$ to $\frac{\norm{u}}{\norm{v}} \cdot v$ is bounded by the distance from $u$ to $v$, plus the distance from $v$ to $\frac{\norm{u}}{\norm{v}} \cdot v$.
		
		\item
		The distance from $u$ to $v$ is bounded as a function of $\varepsilon$, and the distance between $v$ and $\frac{\norm{u}}{\norm{v}} \cdot v$ is bounded by the fact that the norms $\norm{u}$, $\norm{v}$ are very close.
	\end{itemize}

	Formally, assume w.l.o.g. that $u$ is the longer vector between the two, denote the difference vector $r := u - v$ and it follows that $\norm{r} \leq \sqrt{2^n} \cdot \varepsilon$.
	Additionally, from triangle inequality it follows that $\norm{v} \geq \left( \frac{1}{2} - \varepsilon \right) \cdot \sqrt{2^n}$.
	We have te following inequalities.
	
	$$
	\norm{\ket{u} - \ket{v}} =
	\norm{\frac{1}{\norm{u}} \cdot u - \frac{1}{\norm{v}}\cdot v} = 
	\frac{1}{\norm{u}}\cdot \norm{ u - \frac{\norm{u}}{\norm{v}}\cdot v } = 
	$$
	$$
	\frac{1}{\norm{u}}\cdot \norm{ v + r - \frac{\norm{u}}{\norm{v}}\cdot v } \underset{(1)}{\leq}
	\frac{1}{\norm{u}}\cdot \left( \norm{ v - \frac{\norm{u}}{\norm{v}}\cdot v } + \norm{r} \right) \leq
	$$
	$$
	\frac{1}{\norm{u}}\cdot \left( \norm{ v - \frac{\norm{u}}{\norm{v}}\cdot v }  + \varepsilon \cdot \sqrt{2^n} \right) \enspace ,
	$$
	where $(1)$ is due to the triangle inequality.
	
	Next, observe that the ratio $\frac{\norm{u}}{\norm{v}}$ is close to 1: it's at least 1 because we assume that $\norm{u} \geq \norm{v}$, and also,
	$$
	\frac{\norm{u}}{\norm{v}} =
	\frac{\norm{v + r}}{\norm{v}} \leq
	\frac{\norm{v} + \norm{r}}{\norm{v}} \leq
	\frac{\norm{v} + \varepsilon\cdot\sqrt{2^n}}{\norm{v}} = 
	$$
	$$
	1 + \frac{\varepsilon\cdot\sqrt{2^n}}{\norm{v}} \underset{\left( \norm{v} \geq \left( \frac{1}{2} - \varepsilon \right) \cdot \sqrt{2^n} \; , \; \frac{1}{4} \geq \varepsilon \right)}{\leq}
	1 + 4\cdot \varepsilon \enspace ,
	$$
	
	The above implies the following bound,
	$$
	\norm{ v - \frac{\norm{u}}{\norm{v}}\cdot v } = 
	\abs{ 1 - \frac{\norm{u}}{\norm{v}} }\cdot \norm{ v } \leq
	4\cdot \varepsilon \cdot \norm{v} \enspace ,
	$$
	and thus,
	$$
	\frac{1}{\norm{u}}\cdot \left( \norm{ v - \frac{\norm{u}}{\norm{v}}\cdot v }  + \varepsilon \cdot \sqrt{2^n} \right) \leq
	\frac{1}{\norm{u}}\cdot \left( 4\cdot \varepsilon \cdot \norm{v}  + \varepsilon \cdot \sqrt{2^n} \right) = 
	$$
	$$
	\frac{\norm{v}}{\norm{u}}\cdot 4\cdot \varepsilon + \frac{\varepsilon \cdot \sqrt{2^n}}{\norm{u}} \underset{\Big( \substack{\norm{v}\leq \norm{u}, \\ \norm{u} \geq \sqrt{2^n}/2} \Big)}{\leq}
	4\cdot \varepsilon + 2\cdot \varepsilon = 6\cdot \varepsilon \enspace ,
	$$
	that is, $\norm{\ket{u} - \ket{v}} \leq 6\cdot \varepsilon$.
	
	Finally, recall the law of cosines that says that for vectors $x, y$:
	$$
	\norm{x - y}^2 =
	\norm{x}^2 + \norm{y}^2 - 2\cdot\norm{x}\cdot\norm{y}\cdot \cos(\Theta_{x, y}) =
	\norm{x}^2 + \norm{y}^2 - 2\cdot \langle x,y \rangle \enspace ,
	$$
	which implies for unit vectors $\ket{x}, \ket{y}$,
	$$
	\implies \abs{\braket{x}{y}} = \abs{ 1 - \frac{\norm{\ket{x} - \ket{y}}^2}{2} } \enspace .
	$$
	In our case,
	$$
	\abs{\braket{u}{v}} = \abs{ 1 - \frac{\norm{\ket{u} - \ket{v}}^2}{2} } \underset{\left( \substack{\norm{\ket{u} - \ket{v}} \leq 6\cdot \varepsilon, \\ \varepsilon^2 \leq 1/18} \right)}{\geq}
	1 - 18\cdot \varepsilon^2 \enspace .
	$$
		
	$\qed$
\end{proof}

%\begin{lemma}[Probability Mass of Vectors inside Thin Layer is Small] \label{lemma:layer_mass_small}
%	Let $n \in \bbN$, $\secp \in \bbN$ (s.t. $\secp \geq 4$) and denote $\varepsilon := 2^{- n - \secp}$, $N := 2^n$.
%	Then,
%	$$
%	\Pr_{u \gets \normalCompDist^{N}}\left[ \left( \frac{1}{2} - \varepsilon \right)\sqrt{N} \leq \norm{u} < \frac{1}{2}\cdot\sqrt{N} \right] <
%	2^{-\secp}\cdot 6^{-N} \enspace .
%	$$
%\end{lemma}

\subsection{Proof of Lemma \ref{lemma:layer_mass_small}}

\begin{proof}
	Denote $L := \biggl\{ u \in \bbR^{2N} : \left( \frac{1}{2} - \varepsilon \right)\sqrt{N} \leq \norm{u} < \frac{1}{2}\cdot\sqrt{N} \biggr\}$ and by $\mu$ the $2N$-dimensional normal distribution measure, and we have,
	$$
	\Pr_{u \gets \normalCompDist^{N}}\left[ \left( \frac{1}{2} - \varepsilon \right)\sqrt{N} \leq \norm{u} < \frac{1}{2}\cdot\sqrt{N} \right] = 
	$$
	$$
	\Pr_{u \gets \normalDist^{2N}}\left[ \left( \frac{1}{2} - \varepsilon \right)\sqrt{N} \leq \norm{u} < \frac{1}{2}\cdot\sqrt{N} \right] = 
	\mu\left( L \right) \enspace .
	$$
	
	We can bound the measure of $L$ by using the always-increasing exponential function and the multi-dimensional volume of $L$:
	$$
	e^{\left( \frac{1}{4} - \varepsilon \right)N}\cdot \mu\left( L \right) <
	e^{\left( \frac{1}{2} - \varepsilon \right)^2 N}\cdot \mu\left( L \right) =
	\int_{L}e^{\left( \frac{1}{2} - \varepsilon \right)^2 N} \text{d}\mu \leq
	$$
	$$
	\int_{L}e^{\norm{u}^2} \text{d}\mu =
	\int_{L}e^{\norm{u}^2}\cdot e^{-\norm{u}^2/2}\cdot \left( 2\pi \right)^{-N} \text{d}u = 
	\int_{L}e^{\frac{\norm{u}^2 - 2\cdot\ln(2\cdot \pi)N}{2}} \text{d}u < 
	$$
	$$
	\int_{L}e^{\frac{N - 8\cdot\ln(2\cdot \pi)N}{8}} \text{d}u = 
	\int_{L}e^{\frac{1 - 8\cdot\ln(2\cdot \pi)}{8} \cdot N} \text{d}u < 
	e^{-\frac{17}{10} \cdot N}\cdot \int_{L}1\text{d}u = 
	e^{-\frac{17}{10} \cdot N}\cdot \text{Vol}(L) \enspace ,
	$$
	which implies,
	$$
	\mu\left( L \right) <
	e^{-\left( \frac{1}{4} - \varepsilon \right)N}\cdot e^{-\frac{17}{10} \cdot N}\cdot \text{Vol}(L) = 
	e^{- \left( \frac{39}{20} - \varepsilon \right) N} \cdot \text{Vol}(L) \underset{(\varepsilon < 1/20)}{<} 
	e^{- \frac{38}{20} N} \cdot \text{Vol}(L) \enspace ,
	$$
	and it is left to bound the volume of $L$.
	
	The volume of $L$ is a volume that can be calculated rather easily - this is simply the volume of the real sphere $S_{2N}\left(\frac{1}{2}\cdot\sqrt{N}\right)$ of $2N$ dimensions and radius $\frac{1}{2}\cdot\sqrt{N}$, minus the volume of the real sphere $S_{2N}\left( \left( \frac{1}{2} - \varepsilon \right)\sqrt{N} \right)$ of $2N$ dimensions and radius $\left( \frac{1}{2} - \varepsilon \right)\sqrt{N}$.
	Since there are known and convenient formulas for the volume of the $N$-ball, the calculation follows.
	$$
	\text{Vol}(L) = 
	\text{Vol}\left( S_{2N}\left( \frac{1}{2}\cdot \sqrt{N} \right) \right) - 
	\text{Vol}\left( S_{2N}\left( \left( \frac{1}{2} - \varepsilon \right)\sqrt{N} \right) \right) = 
	$$
	$$
	\frac{\pi^{N}}{\Gamma(N + 1)}\cdot \left( \frac{1}{2}\cdot \sqrt{N} \right)^{2N} - \frac{\pi^{N}}{\Gamma(N + 1)}\cdot \left( \left( \frac{1}{2} - \varepsilon \right)\sqrt{N} \right)^{2N} = 
	$$
	$$
	\frac{\pi^{N}\cdot N^N}{N!}\cdot \left( \left( \frac{1}{2} \right)^{2N} - \left( \frac{1}{2} - \varepsilon \right)^{2N} \right) \enspace .
	$$
	
	To bound the above, we'll give a lower bound for $\left( \frac{1}{2} - \varepsilon \right)^{2N}$:
	$$
	\left( \frac{1}{2} - \varepsilon \right)^{2N} = 
	\sum_{i = 0}^{2N} {2N \choose i} (-1)^{i}\cdot \varepsilon^{i}\cdot \frac{1}{2^{2N - i}} =
	$$
	$$
	\frac{1}{2^{2N}} - 2N\varepsilon\cdot \frac{1}{2^{2N - 1}} + \sum_{i = 2}^{2N} {2N \choose i} (-1)^{i}\cdot \varepsilon^{i}\cdot \frac{1}{2^{2N - i}} \underset{(*)}{\geq} 
	\frac{1}{2^{2N}} - 2N\varepsilon\cdot \frac{1}{2^{2N - 1}} \enspace,
	$$
	and we would like to show the inequality $(*)$, that says that the last sum (that sums from $i = 2$ and up) is positive:
	$$
	\sum_{i = 2}^{2N} {2N \choose i} (-1)^{i}\cdot \varepsilon^{i}\cdot \frac{1}{2^{2N - i}} = 
	$$
	$$
	\sum_{i = 2, 4, 6, \cdots, 2N - 2} \left( {2N \choose i}\cdot \varepsilon^{i}\cdot \frac{1}{2^{2N - i}} -
	2\cdot{2N \choose i + 1}\cdot\varepsilon^{i + 1}\cdot \frac{1}{2^{2N - i}} \right) + \varepsilon^{2N} = 
	$$
	$$
	\sum_{i = 2, 4, 6, \cdots, 2N - 2} \left( \varepsilon^{i}\cdot \frac{1}{2^{2N - i}}\cdot \left( {2N \choose i} -  2\cdot{2N \choose i + 1}\cdot\varepsilon \right) \right) + \varepsilon^{2N} \enspace ,
	$$
	and for all $i = 2, 4, 6, \cdots, 2N - 2$ we have,
	$$
	{2N \choose i} -  2\cdot{2N \choose i + 1}\cdot\varepsilon = 
	\prod_{j = 0}^{i - 1}\frac{2N - j}{i - j} - 2\varepsilon\cdot \prod_{j = 0}^{i}\frac{2N - j}{i + 1 - j} = 
	$$
	$$
	\prod_{j = 0}^{i - 1}\frac{2N - j}{i - j} - 2\varepsilon\cdot \left( 2N - i \right) \prod_{j = 0}^{i - 1}\frac{2N - j}{i + 1 - j} \geq
	$$
	$$
	\prod_{j = 0}^{i - 1}\frac{2N - j}{i - j} - 4N\varepsilon\cdot \prod_{j = 0}^{i - 1}\frac{2N - j}{i + 1 - j} \geq
	\left( \prod_{j = 0}^{i - 1}\frac{2N - j}{i - j} \right) \cdot \left( 1 - 4N\varepsilon \right) \underset{(1 \geq 2^{-\secp + 2} = 4N\varepsilon)}{\geq} 0 \enspace.
	$$
	The last inequality implies the inequality $(*)$, which in turn implies the lower bound,
	$$
	\left( \frac{1}{2} - \varepsilon \right)^{2N} \geq 
	\frac{1}{2^{2N}} - 4N\varepsilon\cdot \frac{1}{2^{2N}} \enspace.
	$$
	
	Finally, we obtain the following:
	$$
	\mu\left( L \right) <
	e^{- \frac{38}{20} N} \cdot \text{Vol}(L) = 
	e^{- \frac{38}{20} N} \cdot \frac{\pi^{N}\cdot N^N}{N!}\cdot \left( \left( \frac{1}{2} \right)^{2N} - \left( \frac{1}{2} - \varepsilon \right)^{2N} \right) \leq
	$$
	$$
	e^{- \frac{38}{20} N} \cdot \frac{\pi^{N}\cdot N^N}{N!}\cdot 4N\varepsilon\cdot \frac{1}{2^{2N}} =
	2^{-\secp + 2}\cdot \frac{\pi^{N}\cdot N^N}{e^{\frac{38}{20} N} \cdot 4^{N} \cdot N!} \underset{(\text{Stirling})}{\leq}
	$$
	$$
	2^{-\secp + 2}\cdot \frac{\pi^{N}\cdot N^N}{e^{\frac{38}{20} N} \cdot 4^{N} \cdot \sqrt{2\pi N}\left( \frac{N}{e} \right)^N} = 
	2^{-\secp + 2}\cdot \frac{\pi^{N}}{e^{\frac{18}{20} N} \cdot 4^{N} \cdot \sqrt{2\pi N}} \underset{\left( 6 < e^{\frac{18}{10}} \right)}{<}
	2^{-\secp}\cdot 6^{-N} \enspace .
	$$
	
	$\qed$
\end{proof}

%\begin{corollary}[Balanced Gaussian Vectors are Almost Always Outside of the Thin Layer] \label{cor:balanced_vectors_not_in_layer}
%	Let $n \in \bbN$, $4 \leq \secp \in \bbN$, $\varepsilon := 2^{-n-\secp}$, $B \geq 2\sqrt{n + \secp}$ and let $D$ be the conditional distribution of $u \gets \normalCompDist^{N}$ with the conditions that $\norm{R_{(\varepsilon, B)}(u)} \geq \frac{\sqrt{N}}{2}$ and $\forall i \in [2^n] : |u_i| \leq B$.
%	Then,
%	$$
%	\Pr_{u \gets D}\left[ \norm{u} < \frac{\sqrt{2^n}}{2} \right] < 4\cdot2^{-\secp} \cdot 6^{-2^n} \enspace .
%	$$
%\end{corollary}

\subsection{Proof of Corollary \ref{cor:balanced_vectors_not_in_layer}}

\begin{proof}
	We have,
	$$
	2^{-\secp} \cdot 6^{-2^n} \underset{(\text{Lemma \ref{lemma:layer_mass_small}})}{>}
	\Pr_{u \gets \normalCompDist^{2^n}}\left[ \left( \frac{1}{2} - \varepsilon \right)\sqrt{2^n} \leq \norm{u} < \frac{1}{2}\cdot\sqrt{2^n} \right] \geq 
	$$
	$$
	\Pr_{u \gets \normalCompDist^{2^n}}\left[ \left( \norm{R_{(\varepsilon, B)}(u)} \geq \frac{\sqrt{2^n}}{2} \right) \land \left( \forall i \in [2^n] : |u_i| \leq B \right) \land \left( \norm{u} < \frac{\sqrt{2^n}}{2} \right) \right] = 
	$$
	$$
	\Pr_{u \gets \normalCompDist^{2^n}}\left[ \left( \norm{R_{(\varepsilon, B)}(u)} \geq \frac{\sqrt{2^n}}{2} \right) \land \left( \forall i \in [2^n] : |u_i| \leq B \right) \right] \cdot
	\Pr_{u \gets D}\left[  \norm{u} < \frac{\sqrt{2^n}}{2} \right] \geq
	$$
	$$
	\Pr_{u \gets \normalCompDist^{2^n}}\left[ \left( \norm{u} \geq \frac{\sqrt{2^n}}{2} \right) \land \left( \forall i \in [2^n] : |u_i| \leq B \right) \right] \cdot
	\Pr_{u \gets D}\left[  \norm{u} < \frac{\sqrt{2^n}}{2} \right] \underset{\text{(Corollary \ref{lemma:gaussian_vectors_balanced})}}{>}
	$$
	$$
	\Big( 1 - \left( e^{-\frac{2^n}{4}} + e^{-\secp} \right) \Big) \cdot \Pr_{u \gets D}\left[  \norm{u} < \frac{\sqrt{2^n}}{2} \right] \underset{(2^n \geq 2 \; , \; \secp \geq 3)}{\geq}
	$$
	$$
	\Big( 1 - \left( e^{-\frac{1}{2}} + e^{-3} \right) \Big) \cdot \Pr_{u \gets D}\left[  \norm{u} < \frac{\sqrt{2^n}}{2} \right] >
	\left( \frac{3}{10} \right) \cdot \Pr_{u \gets D}\left[  \norm{u} < \frac{\sqrt{2^n}}{2} \right] \enspace .
	$$
	The above implies in particular,
	$$
	2^{-\secp} \cdot 6^{-2^n} \cdot \left( \frac{10}{3} \right) > \Pr_{u \gets D}\left[  \norm{u} < \frac{\sqrt{2^n}}{2} \right] \enspace ,
	$$
	which implies our wanted inequality.
\end{proof}





